Benchmarking Classical, Deep, and Generative Models for Human Activity Recognition

Human Activity Recognition (HAR) has gained significant importance with the growing use of sensor-equipped devices and large datasets. This paper evaluates the performance of three categories of models : classical machine learning, deep learning architectures, and Restricted Boltzmann Machines (RBMs) using five key benchmark datasets of HAR (UCI-HAR, OPPORTUNITY, PAMAP2, WISDM, and Berkeley MHAD). We assess various models, including Decision Trees, Random Forests, Convolutional Neural Networks (CNN), and Deep Belief Networks (DBNs), using metrics such as accuracy, precision, recall, and F1-score for a comprehensive comparison. The results show that CNN models offer superior performance across all datasets, especially on the Berkeley MHAD. Classical models like Random Forest do well on smaller datasets but face challenges with larger, more complex data. RBM-based models also show notable potential, particularly for feature learning. This paper offers a detailed comparison to help researchers choose the most suitable model for HAR tasks.

==> TABLE.tex <==
\begin{table*}[p]
    \centering
    \normalsize
    \caption{Performance Comparison of Different AI Models for HAR (Part 1)}
    \begin{minipage}{\textwidth}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{p{2.5cm}p{3cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{5cm}}
            \toprule
            Reference & AI Model & Dataset & \multicolumn{4}{c}{Performance} & Findings \\
            & & & Accuracy & F1 Score & Precision & Recall & \\
            \midrule
            Mohamed Abdel-Basset (1) & CNN, T-ResNet, T-DenNet, ResNet & UCI-HAR, WISDM & 96.16\%, 97.24\%, 96.38\%, 98.30\% & - & - & - & Description here. \\
            \midrule
            KUN XIA (5) & CNN, DeepConvLSTM, LSTM-CNN & OPPORTUNITY, WISDM, UCI-HAR & - & - & - & 90.25\%, 92.32\%, 94.75\% & Description here. \\
            \midrule
            Raj Shekhar & Decision Tree, Random Forest, Gradient Boosting Decision Tree, Logistic Regression, Linear SVC, RBF SVM & UCI-HAR & 87\%, 91\%, 95\%, 92\%, 96.50\%, 97\% & - & - & - & Description here. \\
            \bottomrule
        \end{tabular}%
        }
    \end{minipage}

    \begin{minipage}{\textwidth}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{p{2.5cm}p{3cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{5cm}}
            \toprule
            Reference & AI Model & Dataset & \multicolumn{4}{c}{Performance} & Findings \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \bottomrule
        \end{tabular}%
        }
    \end{minipage}
    \label{tab:performance_comparison}
\end{table*}


==> TABLE2.tex <==
\begin{table*}[p]
    \centering
    \normalsize
    \caption{Performance Comparison of Different AI Models for HAR (Part 1)}
    \begin{minipage}{\textwidth}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{p{2.5cm}p{3cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{5cm}}
            \toprule
            Reference & AI Model & Dataset & \multicolumn{4}{c}{Performance} & Findings \\
            & & & Accuracy & F1 Score & Precision & Recall & \\
            \midrule
            Mohamed Abdel-Basset (1) & CNN, T-ResNet, T-DenNet, ResNet & UCI-HAR, WISDM & 96.16\%, 97.24\%, 96.38\%, 98.30\% & - & - & - & Description here. \\
            \midrule
            KUN XIA (5) & CNN, DeepConvLSTM, LSTM-CNN & OPPORTUNITY, WISDM, UCI-HAR & - & - & - & 90.25\%, 92.32\%, 94.75\% & Description here. \\
            \midrule
            Raj Shekhar & Decision Tree, Random Forest, Gradient Boosting Decision Tree, Logistic Regression, Linear SVC, RBF SVM & UCI-HAR & 87\%, 91\%, 95\%, 92\%, 96.50\%, 97\% & - & - & - & Description here. \\
            \bottomrule
        \end{tabular}%
        }
    \end{minipage}

    \begin{minipage}{\textwidth}
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{p{2.5cm}p{3cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}p{5cm}}
            \toprule
            Reference & AI Model & Dataset & \multicolumn{4}{c}{Performance} & Findings \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \midrule
            LIMENG LU (55) & Multichannel CNN-GRU & WISDM, UCI-HAR, PAMAP2 & 96.41\%, 96.67\%, 96.25\% & - & - & - & Description here. \\
            \midrule
            Nidhi Dua (56) & Multi-input CNN-GRU & UCI-HAR, WISDM, PAMAP2 & 96.20\%, 97.21\%, 95.27\% & - & - & - & Description here. \\
            \bottomrule
        \end{tabular}%
        }
    \end{minipage}
    \label{tab:123}
\end{table*}

